Space-Variant Total Variation boosted by learning techniques in few-view tomographic imaging

This paper focuses on the development of a space-variant regularization model for solving an under-determined linear inverse problem. The case study is a medical image reconstruction from few-view tomographic noisy data. The primary objective of the proposed optimization model is to achieve a good balance between denoising and the preservation of fine details and edges, overcoming the performance of the popular and largely used Total Variation (TV) regularization through the application of appropriate pixel-dependent weights. The proposed strategy leverages the role of gradient approximations for the computation of the space-variant TV weights. For this reason, a convolutional neural network is designed, to approximate both the ground truth image and its gradient using an elastic loss function in its training. Additionally, the paper provides a theoretical analysis of the proposed model, showing the uniqueness of its solution, and illustrates a Chambolle-Pock algorithm tailored to address the specific problem at hand. This comprehensive framework integrates innovative regularization techniques with advanced neural network capabilities, demonstrating promising results in achieving high-quality reconstructions from low-sampled tomographic data.

==> convergence_FULL.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
%%%%%%%%%%%%%%%%%%%%%%%     \subsection{Convergence theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  


Now, after having demonstrated that $\x^*_{\Psi, \delta}$ is well-defined (as it is unique for any fixed $\delta>0$ and any reconstructor $\Psi$), we investigate some convergence features of the proposed weighted space-variant regularization model stated in Definition \ref{def:NostroMinimo}. 
In the following, with a minor notational adaptation, we use $\x^*_{GT, \delta}$ to indicate the solution of the $\Psi$-W$\ell_1$ algorithm when $\tilde{\x} = \x^{GT}$. Similarly, we set:
\begin{align}\label{eq:J_GT}
    \mathcal{J}_{GT}(\x, \y^\delta) :=  ||\K\x, \y^\delta||_2^2 + \lambda || \w_\eta(\x^{GT}) \odot | \D \x | ||_1.
\end{align}
In  Section \ref{ssec:OurModel}, we have already intuitively observed that $\x^{GT}$ would be a clever candidate as $\tilde\x$, and the closer $\w_\eta(\tilde{\x})$ is to $\w_\eta(\x^{GT})$, the higher the reconstruction quality achieved by the $\Psi$-W$\ell_1$ algorithm will be. In particular, since $\w_\eta(\x)$ only depends on the gradient magnitude of $\x$, we expect that the reconstruction error will be related to the distance between $| \D \x^{GT} |$ and $| \D \tilde{\x} |$.  
In addition, for a fixed noise norm $\delta > 0$, the $\Psi$-W$\ell_1$ method is optimal whenever $\tilde{\x} = \x^{GT}$, that is when its solution is $\x^*_{GT, \delta}$. 

% *********************** PSI vs GT\\
In the following, we prove a stability result showing that $|| \x^*_{GT, \delta} - \x^*_{\Psi, \delta} ||_1$, i.e. the error introduced by using $\Psi(\y^\delta)$ instead of $\x^{GT}$ to define $\w_\eta(\tilde{\x})$ in the objective function $\mathcal{J}$, converges to $0$ as the distance $|| \Psi(\y^\delta) - \x^{GT} ||_1$ goes to 0.
To this aim, we illustrate the concepts of $p$-norm accuracy $\eta_p^{-1}$ and $p$-norm $\epsilon$-stability constant $C^\epsilon_{\Psi, p}$ of a reconstructor $\Psi$, generalizing the definitions in \cite{evangelista2022or,evangelista2023ambiguity}.

\begin{definition}\label{def:accuracy}
    Let $\Psi: \R^m \to \R^n$ be a reconstructor. Let:
    \begin{align*}
        \eta_p = \sup_{\x \in \X} || \Psi(\K \x) - \x ||_p < \infty.
    \end{align*}
    If $\eta_p < \infty$, we say the $\Psi$ is $\eta_p^{-1}$-accurate in $p$-norm.
\end{definition}

\begin{definition}\label{def:stability_constant}
    Let $\Psi: \R^m \to \R^n$ be an $\eta_p^{-1}$-accurate reconstructor in $p$-norm. Then, for any $\epsilon > 0$, we say that $C^\epsilon_{\Psi, p}$ is the $p$-norm $\epsilon$-stability constant if:
    \begin{align*}
        C^\epsilon_{\Psi, p} = \sup_{\substack{\x \in \X \\ || \e ||_p \leq \epsilon}} \frac{|| \Psi(\K\x + \e) - \x ||_p - \eta_p}{|| \e ||_p}.
    \end{align*}
\end{definition}
For an analysis of the accuracy and the stability constant of a reconstructor, see \cite{evangelista2022or} where the case $p=2$ is explored in detail. Note that most of the results obtained for $p=2$ can be easily extended to $p\geq 1$. 
In the context of this study, we emphasize that $\eta_p$ delineates the upper bound on the reconstruction error (measured in the $p$-norm) incurred by the reconstructor $\Psi$ when applied to noiseless data (when $\delta=0$). Conversely, $C^\epsilon_{\Psi, p}$ serves as a metric quantifying the amplification (or reduction), provided by $\Psi$, of input noise, which is upper bounded within a $p$-norm by $\epsilon$ in the data,  % For the scope of this work, we need to highlight that $\eta_p$ describes the maximum reconstruction error (in $p$-norm) committed by the reconstructor $\Psi$ when applied to noiseless data, while $C^\epsilon_{\Psi, p}$ quantifies how much the input noise (with $p$-norm bounded by $\epsilon$) corrupting the data gets amplified (or reduced) by the reconstructor. This can be easily seen by observing that 
since Definition \ref{def:stability_constant} can be rewritten as:
\begin{align}\label{eq:consequence_stab_constant}
    || \Psi(\K\x + \e) - \x ||_p \leq \eta_p + C^\epsilon_{\Psi, p} ||\e ||_p, \quad \forall \: || \e ||_p \leq \epsilon, \: \x \in \X.
\end{align} 

% to estimate  $|| \x^*_{GT, \delta} - \x^*_{\Psi, \delta} ||_1$, i.e. the error introduced by using $\Psi(\y^\delta)$ instead of $\x^{GT}$ to define $\w^\delta_\eta(\tilde{\x})$, with a constant depending on $\w$, $\eta_1$ and $C^\epsilon_{\Psi, 1}$, where $\epsilon$ is the maximum norm of the noise, a quantity related to $\delta$. 
Now, we need to prove a couple of results.  
\begin{proposition}\label{prop:lip_of_w}
    % Let:
    % \begin{align}
    %     \w^\delta_\eta(\tilde{\x}) =  \left( \frac{\eta}{\sqrt{\eta^2 + | \D\tilde{\x} |^2}} \right)^{1-p}.
    % \end{align}     Then 
    For any $\delta > 0$ and any $\eta > 0$, $\w_\eta(\tilde{\x})$ defined in Equation \eqref{eq:OurWeights} is a Lipschitz continuous function of $| \D\tilde{\x} |$ in 1-norm, i.e. for any $\tilde{\x}, \tilde{\x}' \in \X$, there exists $L(\w_\eta) \geq0$ such that:
    \begin{align*}
        || \w_\eta(\tilde \x) - \w_\eta(\tilde{\x}') ||_1 \leq L(\w_\eta) || | \D \tilde{\x} | - | \D \tilde{\x}' | ||_1.
    \end{align*}
\end{proposition}

\begin{proof}
    If we consider:
    \begin{align*}
        f(\alpha) = \left( \frac{\eta}{\sqrt{\eta^2 + \alpha^2}} \right)^{1-p},
    \end{align*}
    the proof trivially follows from the observation that $f'(\alpha)$ is a continuous function of $\alpha$. Indeed:
    \begin{align*}
        f'(\alpha) =  (p-1) \frac{\alpha}{\sqrt{\eta^2 + \alpha^2}} \left( \frac{\eta}{\sqrt{\eta^2 + \alpha^2}} \right)^{p-2},
    \end{align*}
    which is continuous everywhere if $\eta \neq 0$.
\end{proof}

\begin{proposition}\label{prop:distance_of_J}
    For any $\x \in \X$, any fixed $\delta > 0$ and any $\y^\delta \in \R^m$, it holds:
    \begin{align}
        | \mathcal{J}_{GT}(\x, \y^\delta) -\mathcal{J}(\x, \y^\delta) | \leq L(\w_\eta) || \D ||_{2, 1} \left( \eta_1 + C^\epsilon_{\Psi, 1} ||\e||_1 \right) || \D \x ||_{2, 1},
    \end{align}
    where $\eta_1$ and $C^\epsilon_{\Psi, 1}$ are the accuracy and the $\epsilon$-stability constant in 1-norm of $\Psi$, respectively,  $\epsilon>0$ is the maximum expected noise norm in $\y^\delta$, and $\mathcal{J}_{GT}$ is given by Equation \eqref{eq:J_GT}.
\end{proposition}

\begin{proof}
    We first note that:
    \begin{align*}
        \mathcal{J}_{GT}(\x, \y^\delta) -\mathcal{J}(\x, \y^\delta)  
        =
        || \w_\eta(\x^{GT}) \odot | \D \x | ||_1 - || \w_\eta(\Psi(\y^\delta)) \odot | \D \x | ||_1.
    \end{align*}
    Thus,
    \begin{align*}
        | 	\mathcal{J}_{GT}(\x, \y^\delta) -\mathcal{J}(\x, \y^\delta) | & 
        = |\ || \w_\eta(\x^{GT}) \odot | \D \x | ||_1 - || \w_\eta(\Psi(\y^\delta)) \odot | \D \x | ||_1 \ | \\
        &
        \leq|| \w_\eta(\x^{GT}) \odot | \D \x | - \w_\eta(\Psi(\y^\delta)) \odot | \D \x | ||_1
    \end{align*}
    by the reverse triangular inequality.\\
    %
    Now, let $\boldsymbol{W}_\eta(\tilde{\x})$ be the $n \times n$ diagonal matrix, whose diagonal entries are the elements of $\w_\eta(\tilde{\x})$, so that $\w_\eta(\tilde{\x}) \odot | \D \x | = \boldsymbol{W}_\eta(\tilde{\x}) | \D \x |$.
    Consequently, it holds:
    \begin{align*}
            | 	\mathcal{J}_{GT}(\x, \y^\delta) -\mathcal{J}(\x, \y^\delta) |
            &
            \leq \left\| \boldsymbol{W}_\eta(\x^{GT}) | \D \x | - \boldsymbol{W}_\eta(\Psi(\y^\delta))  | \D \x | \right\|_1 \\ 
            &
            = \left\| \left( \boldsymbol{W}_\eta(\x^{GT}) - \boldsymbol{W}_\eta(\Psi(\y^\delta)) \right) | \D \x |  \right\|_1 \\ 
            &
            \leq \left\| \boldsymbol{W}_\eta(\x^{GT}) - \boldsymbol{W}_\eta(\Psi(\y^\delta))  \right\|_1 \left\| | \D \x | \right\|_1.
    \end{align*}
    From Proposition \ref{prop:lip_of_w}, it follows:
    \begin{align*}
        \left\| \boldsymbol{W}_\eta(\x^{GT}) - \boldsymbol{W}_\eta(\Psi(\y^\delta))  \right\|_1 
        \leq 
        L(\w_\eta) \left\| | \D \x^{GT} | - | \D \Psi(\y^\delta) | \right\|_1,
    \end{align*}
    where $L(\w_\eta)$ is the Lipschitz constant of $\w_\eta$.
    
    To go on, note that the triangular inequality gives:
    \begin{align*}
        \left\| | \D \x^{GT} | - | \D \Psi(\y^\delta) | \right\|_1 
        \leq 
        \left\| |  \D \x^{GT} - \D \Psi(\y^\delta)  | \right\|_1
        = 
        \left\| \D \left(\x^{GT} -\Psi (\y^\delta)\right) \right\|_{2,1},
    \end{align*}
    where $|| \cdot ||_{2, 1}$ is defined in \eqref{eq:TV_definition}. Now, let $|| \D ||_{2, 1}$ be the matrix norm induced by the $|| \cdot ||_{2, 1}$ vector norm, i.e.:
    \begin{align*}
        || \D ||_{2, 1} := \max_{\x \in \R^n} \frac{|| \D \x ||_{2, 1}}{|| \x ||_1}.
    \end{align*}
    We get:
    \begin{align*}
        || \D \left(\x^{GT} -\Psi (\y^\delta)\right) ||_{2,1} \leq || \D ||_{2, 1} || \x^{GT} - \Psi(\y^\delta) ||_1.
    \end{align*}
    To conclude, let $\epsilon > 0$ be the maximum expected norm of $\e$ in $\y^\delta = \K \x^{GT} + \e$. By Equation \eqref{eq:consequence_stab_constant}, following from Definition \ref{def:stability_constant}:
    \begin{align*}
        || \x^{GT} - \Psi(\y^\delta) ||_1 = || \x^{GT} - \Psi(\K \x^{GT} + \e) ||_1 \leq \eta_1 + C^\epsilon_{\Psi, 1} || \e ||_1,
    \end{align*}
    where $\eta_1$ and $C^\epsilon_{\Psi, 1}$ are the accuracy and the $\epsilon$-stability constant in 1-norm of $\Psi$, respectively.
    Synthesizing these findings, we get:
    \begin{align*}
        | 	\mathcal{J}_{GT}(\x, \y^\delta) -\mathcal{J}(\x, \y^\delta) | \leq L(\w_\eta) || \D ||_{2, 1} \left( \eta_1 + C^\epsilon_{\Psi, 1} ||\e||_1 \right) \left\| | \D \x | \right\|_1,
    \end{align*}
    which proves the result.
\end{proof}

In the remainder of this Section, we prove that
\begin{align*}
    || \x^*_{GT, \delta} - \x^*_{\Psi, \delta} ||_1 \to 0, \mbox{ as } || \Psi(\y^\delta) - \x^{GT} ||_1 \to 0.
\end{align*}
We require a preliminary result.
\begin{proposition}\label{prop:uniformconvergence_implies_convergenceminimizers}
    Let $\{ f_k \}_{k \in \mathbb{N}}$ be a sequence of functions and assume that $f_k$ converges uniformly to $f^*$ on any compact subset of $\X$. Then, if for any $k \in \mathbb{N}$, the problem:
    \begin{align*}
        \min_{\x \in \X} f_k(\x),
    \end{align*}
    has a unique solution $\x_k$, and:
    \begin{align*}
        \min_{\x \in \X} f^*(\x),
    \end{align*}
    has a unique solution $\x^*$, then:
    \begin{align*}
        \lim_{k \to \infty} || \x_k - \x^* ||_1 = 0.
    \end{align*}
\end{proposition}

\begin{proof}
    Let $\x_k$ be the unique minimizer of $f_k$ for any $k \in \mathbb{N}$ and let $C \subseteq \X$ any compact set such that $\x_k \in C$ for any $k \in \mathbb{N}$. Since $\{ \x_k \}_{k \in \mathbb{N}}$ is a sequence in a compact set, there exists a convergent subsequence $\{ \x_{k_j} \}_{j \in \mathbb{N}}$. Let $\x^*$ be the limit of this subsequence. By definition, for any $k \in \mathbb{N}$, it holds:
    \begin{align*}
        f_k(\x_k) \leq f_k(\x), \quad \forall \x \in C,
    \end{align*}
    and in particular:
    \begin{align*}
        f_{k_j}(\x_{k_j}) \leq f_{k_j}(\x), \quad \forall \x \in C.
    \end{align*}
    Since $f_k$ converges uniformly to $f^*$ and $\x_{k_j}$ converges to $\x^*$, it holds that:
    \begin{align*}
        &\lim_{j \to \infty} f_{k_j}(\x_{k_j}) = f^*(\x^*), \\
        &\lim_{j \to \infty} f_{k_j}(\x) = f^*(\x), \quad \forall \x \in C.
    \end{align*}
    Consequently,
    \begin{align*}
        f^*(\x^*) \leq f^*(\x), \quad \forall \x \in C,
    \end{align*}
    i.e. $\x^*$ is a minimizer of $f^*$. Since $f^*$ has a unique minimizer, then all the subsequences of $\x_k$ converge to the same element $\x^*$, which implies that $\x_k$ converges to $\x^*$ as $k \to \infty$. In particular:
    \begin{align*}
        \lim_{k \to \infty} || \x_k - \x^* ||_1 = 0.
    \end{align*}
\end{proof}

To proceed, we first consider the noiseless case (i.e. $\delta = 0$), for which it holds the following Proposition.

\begin{proposition}\label{prop:stability_delta0}
    Let $\x^*_{GT, 0}$ be the unique minimum of $\mathcal{J}_{GT}(\x, \y^\delta)$, defined in \eqref{eq:J_GT}, with $\delta = 0$. Let $\{ \Psi_k \}_{k \in \mathbb{N}}$ be a sequence of reconstructor with 1-accuracy $\eta_{1, k}^{-1}$ for any $k \in \mathbb{N}$. Let $\x^*_{k, 0}$ be the unique minimum of $\mathcal{J}_k(\x, \y^0) := \mathcal{J}(\x, \y^\delta)$ with $\Psi = \Psi_k$ and $\delta = 0$. Then, if $\eta_{1, k} \to 0$ for $k \to \infty$:
    \begin{align*}
        || \x^*_{GT, 0} - \x^*_{k, 0} ||_1 \to 0.
    \end{align*}
\end{proposition}

\begin{proof}
    If $\delta = 0$, then for any $k \in \mathbb{N}$, Proposition \ref{prop:distance_of_J} implies:
    \begin{align*}
        | \mathcal{J}_{GT}(\x, \y^0) - \mathcal{J}_k(\x, \y^0) | \leq \eta_{1, k} L(\w_\eta) || \D ||_{2, 1} || \D \x ||_{2, 1} &\leq \eta_{1, k} L(\w_\eta) || \D ||_{2, 1}^2 || \x ||_1 \\ &\leq \eta_{1, k} n L(\w_\eta) || \D ||_{2, 1}^2 || \x ||_{\infty}, 
    \end{align*}
    which, considering that $\eta_{1, k} \to 0$ as $k \to \infty$, implies that $\mathcal{J}_k(\x, \y^0) \to \mathcal{J}_{GT}(\x, \y^0)$ uniformly on every compact subset of $\X$. \\
    
    Let $C \subseteq \X$ be the closure of any set that contains $\x^*_{k, 0}$ for all $k \in \mathbb{N}$. Note that $C$ is limited, indeed let $\x^\dagger \in \R^n$ be a solution of $\K \x = \y^0$, then for any $k \in \mathbb{N}$:
    \begin{align*}
        \lambda || \w_\eta(\Psi_k(\y^0)) \odot | \D \x^*_{k, 0} | ||_1 \leq \mathcal{J}_k(\x^*_k, \y^0) \leq \mathcal{J}_k(\x^\dagger, \y^0) = \lambda || \w_\eta(\Psi_k(\y^0)) \odot | \D \x^\dagger | ||_1,
    \end{align*}
    where the second inequality comes from the definition of minimizer. By Proposition \ref{prop:w_is_a_scale_term} $\w_\eta(\Psi_k(\y^0)) \leq \boldsymbol{1}$, thus:
    \begin{align*}
        \lambda || \w_\eta(\Psi_k(\y^0)) \odot | \D \x^*_{k, 0} | ||_1 \leq \lambda || \w_\eta(\Psi_k(\y^0)) \odot | \D \x^\dagger | ||_1 \leq \lambda || \D\x^\dagger ||_{2, 1} = c < \infty.
    \end{align*}
    Consequently,
    \begin{align*}
        \lim_{k \to \infty} \lambda || \w_\eta(\Psi_k(\y^0)) \odot | \D \x^*_{k, 0} | ||_1 < \infty,
    \end{align*}
    which, since $\lambda || \w_\eta(\Psi_k(\y^0)) \odot | \D \x^*_{k, 0} | ||_1$ is coercive, implies that $\{ \x_k \}_{k \in \mathbb{N}}$ is limited, and so is $C$. \\
    
    Since $C$ is closed and limited, it is compact, and thus $\mathcal{J}_k(\x, \y^0) \to \mathcal{J}_{GT}(\x, \y^0)$ uniformly in $C$. Since uniform convergence implies convergence of the minimum, since $\x^*_{k, 0}$ is unique by Theorem \ref{theo:unicita}, $|| \x^*_{k, 0} - \x^*_{GT, 0} ||_1 \to 0$ as $k \to \infty$.
\end{proof}

We can also prove a convergence result for $\x^*_{GT, \delta}$ and $\x^*_{\Psi, \delta}$.
\begin{proposition}\label{prop:convergence_GT}
    Let $\{ \delta_k \}_{k \in \mathbb{N}}$ be any sequence of positive noise levels such that $\delta_k \to 0$ as $k \to \infty$. For any $k \in \mathbb{N}$, let $\x^*_{GT, \delta_k}$ be the unique minimizer of $\mathcal{J}_{GT}(\x, \y^{\delta_k})$. Then:
    \begin{align*}
        \lim_{k \to \infty} || \x^*_{GT, \delta_k} - \x^*_{GT, 0} ||_1 \to 0.
    \end{align*}
\end{proposition}

\begin{proof}
    Note that $\mathcal{J}_{GT}(\x, \y^{\delta_k})$ is continuous with respect to $\y^{\delta_k}$, since the term $\y^{\delta_k}$ appears in $\mathcal{J}_{GT}(\x, \y^{\delta_k})$ only via a quadratic term. Consequently,
    \begin{align}
        \lim_{k \to \infty} \mathcal{J}_{GT}(\x, \y^{\delta_k}) = \mathcal{J}_{GT}(\x, \y^{0}), \quad \forall \x \in \X.
    \end{align}
    To prove the result, we need to show that $\mathcal{J}_{GT}(\x, \y^{\delta_k})$ converges uniformly to $\mathcal{J}_{GT}(\x, \y^{0})$ in $\x$ which, together with the unicity of the minimizes, implies that $\x^*_{GT, \delta_k}$ converges to $\x^*_{GT, 0}$ as $k \to \infty$. To this aim, note that for any $\x \in \X$:
    \begin{align*}
        \left| \mathcal{J}_{GT}(\x, \y^{\delta_k}) - \mathcal{J}_{GT}(\x, \y^{0}) \right| &=\left| \frac{1}{2}|| \K \x - \y^{\delta_k} ||_2^2 -  \frac{1}{2}|| \K \x - \y^{0} ||_2^2 \right| \\ &\leq \frac{1}{2}||  \K \x - \y^{\delta_k} - \left( \K \x - \y^0 \right) ||_2^2 \\ & = \frac{1}{2}|| \y^{\delta_k} - \y^0 ||_2^2 \leq \frac{1}{2}\delta_k^2.
    \end{align*}
    Since $\delta_k$ does not depend on $\x$, and $\delta_k \to 0$ as $k \to \infty$, then this implies that $\mathcal{J}_{GT}(\x, \y^{\delta_k})$ converges to $\mathcal{J}_{GT}(\x, \y^{0})$ uniformly, thus $\x^*_{GT, \delta_k}$ converges to $\x^*_{GT, 0}$ and, in particular,
    \begin{align*}
        \lim_{k \to \infty}|| \x^*_{GT, \delta_k} - \x^*_{GT, 0} ||_1 = 0.
    \end{align*}
\end{proof}

The convergence of $\x^*_{\Psi, \delta}$ to $\x^*_{\Psi, 0}$ as $\delta \to 0$ for a general reconstructor $\Psi$ is slightly harder, since in this case, the regularizer also depends on $\delta$ due to $\tilde{\x} = \Psi(\y^\delta)$. 

\begin{proposition}\label{prop:convergence_Psi}
    For any reconstructor $\Psi: \R^m \to \R^n$, let $\{ \delta_k \}_{k \in \mathbb{N}}$ be any sequence of positive noise levels such that $\delta_k \to 0$ as $k \to \infty$. For any $k \in \mathbb{N}$, let $\x^*_{\Psi, \delta_k}$ be the unique minimizer of $\mathcal{J}_{\Psi}(\x, \y^{\delta_k})$. Then:
    \begin{align*}
        \lim_{k \to \infty} || \x^*_{\Psi, \delta_k} - \x^*_{\Psi, 0} ||_1 \to 0.
    \end{align*}
\end{proposition}

\begin{proof}
    We proceed as in the proof of Proposition \ref{prop:convergence_GT}. 
    \begin{align*}
        \left| \mathcal{J}_{\Psi}(\x, \y^{\delta_k}) - \mathcal{J}_{\Psi}(\x, \y^{0}) \right| &= \left| \frac{1}{2}|| \K \x - \y^{\delta_k} ||_2^2 -  \frac{1}{2}|| \K \x - \y^{0} ||_2^2 + \lambda \left( \mathcal{R}_k(\x) - \mathcal{R}_0(\x) \right) \right| \\ &\leq \left| \frac{1}{2}|| \K \x - \y^{\delta_k} ||_2^2 -  \frac{1}{2}|| \K \x - \y^{0} ||_2^2 \right| + \lambda \left| \mathcal{R}_k(\x) - \mathcal{R}_0(\x) \right| \\ &\leq \frac{1}{2}\delta_k^2 + \lambda \left| \mathcal{R}_k(\x) - \mathcal{R}_0(\x) \right|,
    \end{align*}
    where for simplicity we denoted as $\mathcal{R}_k(\x)$ the value of the regularizer with weights computed by $\Psi(\y^{\delta_k})$, i.e. $\mathcal{R}_k(\x) = || \w_\eta(\Psi(\y^{\delta_k})) \odot | \D \x | ||_1$. By Proposition \ref{prop:lip_of_w},
    \begin{align*}
        \left| \mathcal{R}_k(\x) - \mathcal{R}_0(\x) \right| &= \left| || \w_\eta(\Psi(\y^{\delta_k})) \odot | \D \x | ||_1 - ||\w_\eta(\Psi(\y^{0})) \odot | \D \x | ||_1 \right| \\ & \leq || \w_\eta(\Psi(\y^{\delta_k})) \odot | \D \x | - \w_\eta(\Psi(\y^{0})) \odot | \D \x | ||_1 \\ &= || \left(\w_\eta(\Psi(\y^{\delta_k})) - \w_\eta(\Psi(\y^{0}))\right) \odot | \D \x | ||_1 \\ &\leq || \w_\eta(\Psi(\y^{\delta_k})) - \w_\eta(\Psi(\y^{0})) ||_1 || \D \x ||_{2,1} \\ &\leq || \w_\eta(\Psi(\y^{\delta_k})) - \w_\eta(\Psi(\y^{0})) ||_1 || \D ||_{2,1} || \x ||_1 \\ &\leq || \w_\eta(\Psi(\y^{\delta_k})) - \w_\eta(\Psi(\y^{0})) ||_1 || \D ||_{2,1} n || \x ||_\infty \\ &\leq L(\w_\eta) || \Psi(\y^{\delta_k}) - \Psi(\y^0)||_1 || \D ||_{2,1} n || \x ||_\infty \\ &\leq L(\w_\eta) L(\Psi) || \D ||_{2,1} n || \x ||_\infty,
    \end{align*}
    where $L(\Psi)$ is the Lipschitz constant of $\Psi$, which is well defined since $\Psi$ is Lipschitz continuous by definition.

    To summarize, we proved that:
    \begin{align*}
        \left| \mathcal{J}_{\Psi}(\x, \y^{\delta_k}) - \mathcal{J}_{\Psi}(\x, \y^{0}) \right| \leq \frac{1}{2}\delta_k^2 + \lambda L(\w_\eta) L(\Psi) || \D ||_{2,1} n || \x ||_\infty,
    \end{align*}
    which implies that $\mathcal{J}_{\Psi}(\x, \y^{\delta_k})$ converges uniformly to $\mathcal{J}_{\Psi}(\x, \y^{0})$ on any compact subset of $\X$. By considering the closed subset $C$ of $\X$ that contains the sequence $\{ \x^*_{\Psi, \delta_k} \}_{k \in \mathbb{N}}$, we conclude as in Proposition \ref{prop:convergence_GT}, by observing that $C$ is limited since:
    \begin{align*}
        || \w_\eta(\Psi(\y^{\delta_k})) \odot | \D \x^*_{\Psi, \delta_k} | ||_1 &\leq \mathcal{J}_\Psi(\x^*_{\Psi, \delta_k}, \y^{\delta_k}) \leq \mathcal{J}_\Psi(\x^\dagger, \y^{\delta_k}) \\ & \leq \frac{\delta_k^2}{2} + || \w_\eta(\Psi(\y^{\delta_k})) \odot | \D \x^\dagger | ||_1 \leq \leq \frac{\delta_k^2}{2} + || \D \x^\dagger ||_{2, 1} \to c < \infty,
    \end{align*}
    and $|| \w_\eta(\Psi(\y^{\delta_k})) \odot | \D \x^*_{\Psi, \delta_k} | ||_1$ is coercive.
\end{proof}

To conclude this Section, we observe that the stability results from Proposition \ref{prop:stability_delta0} can be generalized to the case where $\delta > 0$. 

\begin{theorem}
    Given $\delta > 0$, let $\{ \Psi_k \}_{k \in \mathbb{N}}$ be a sequence of reconstructor such that:
    \begin{align*}
        \lim_{k \to \infty} || | \D\Psi_k(\y^\delta)| - | \D\x^{GT}| ||_1 = 0, \quad \forall \y^\delta = \K\x^{GT} + \e, || \e ||_2 \leq \delta,
    \end{align*}
    then:
    \begin{align*}
        \lim_{k \to \infty} || \x^*_{GT, \delta} - \x^*_{\Psi_k, \delta} ||_1 = 0.
    \end{align*}
\end{theorem}

\begin{proof}
    Let:
    \begin{align*}
        \mathcal{J}_k(\x, \y^\delta) := \frac{1}{2} || \K\x - \y^\delta ||_2^2 + \lambda || \w_\eta(\Psi_k(\y^\delta)) \odot | \D \x | ||_1.
    \end{align*}
    By proceeding as in the proof of Proposition \ref{prop:distance_of_J}, we can prove that:
    \begin{align*}
        | \mathcal{J}_k(\x, \y^\delta) - \mathcal{J}_{GT}(\x, \y^\delta) | \leq L(\w_\eta) \left\| | \D \x^{GT} | - | \D \Psi_k(\y^\delta) | \right\|_1 || \D \x ||_{2, 1},
    \end{align*}
    where $L(\w_\eta)$ is defined as in Proposition \ref{prop:lip_of_w}. Consequently:
    \begin{align*}
        | \mathcal{J}_k(\x, \y^\delta) - \mathcal{J}_{GT}(\x, \y^\delta) | &\leq n L(\w_\eta) || \D ||_{2, 1} || \x ||_\infty \left\| | \D \x^{GT} | - | \D \Psi_k(\y^\delta) | \right\|_1,
    \end{align*}
    which implies that $\mathcal{J}_k(\x, \y^\delta)$ converges to $\mathcal{J}_GT(\x, \y^\delta)$ uniformly on any compact, whenever
    \begin{align*}
        \lim_{k \to \infty} \left\| | \D \x^{GT} | - | \D \Psi_k(\y^\delta) | \right\|_1 = 0.
    \end{align*}
    By Proposition \ref{prop:uniformconvergence_implies_convergenceminimizers}, we conclude that:
    \begin{align*}
        \lim_{k \to \infty} || \x^*_{GT, \delta} - \x^*_{\Psi_k, \delta} ||_1 = 0.
    \end{align*}
\end{proof}
% \begin{theorem}
%     There exist three functions, $\mathcal{E}_{GT}(\delta)$, $\mathcal{E}^1_{\Psi}(\delta)$ and $\mathcal{E}^2_\Psi(\eta_1)$, such that:
%     \begin{align*}
%         & \lim_{\delta \to 0} \mathcal{E}_{GT}(\delta) = 0, \\
%         & \lim_{\delta \to 0} \mathcal{E}^1_{\Psi}(\delta) = 0, \\
%         & \lim_{\eta_1 \to 0} \mathcal{E}^2_{\Psi}(\eta_1) = 0,
%     \end{align*}
%     for which it holds:
%     \begin{align}
%         || \x^*_{GT, \delta} - \x^*_{\Psi, \delta} ||_1 \leq \mathcal{E}_{GT}(\delta) + \mathcal{E}^1_{\Psi}(\delta) + \mathcal{E}^2_\Psi(\eta_1).
%     \end{align}
%     % Let $\{ \Psi_k \}_{k \in \mathbb{N}}$ be a sequence of reconstructor with 1-accuracy $\eta_{1, k}^{-1}$ for any $k \in \mathbb{N}$. Let $\x^*_{k, \delta}$ be the unique minimum of $\mathcal{J}_k(\x, \y^\delta) := \mathcal{J}(\x, \y^\delta)$ with $\Psi = \Psi_k$. Then, if $\eta_k \to 0$ for $k \to \infty$:
%     % \begin{align*}
%     %     || \x^*_{GT, \delta} - \x^*_{k, \delta} ||_1 \to 0.
%     % \end{align*}
% \end{theorem}

% \begin{proof}
%     From the triangular inequality:
%     \begin{align*}
%         || \x^*_{GT, \delta} - \x^*_{\Psi, \delta} ||_1 \leq || \x^*_{GT, \delta} - \x^*_{GT, 0} ||_1 + || \x^*_{\Psi, \delta} - \x^*_{\Psi, 0} ||_1 + || \x^*_{GT, 0} - \x^*_{\Psi, 0} ||_1. 
%     \end{align*}
%     Proposition \ref{prop:convergence_GT} implies that, for any $\delta > 0$, there exists $\mathcal{E}_{GT}(\delta) > 0$ such that $|| \x^*_{GT, \delta} - \x^*_{GT, 0} ||_1 < \mathcal{E}_{GT}(\delta)$. Similarly, from Proposition \ref{prop:convergence_Psi}, for any $\delta > 0$, there exists $\mathcal{E}^1_{\Psi}(\delta) > 0$ such that $|| \x^*_{\Psi, \delta} - \x^*_{\Psi, 0} ||_1 < \mathcal{E}^1_{\Psi}(\delta)$. Again, from Proposition \ref{prop:stability_delta0}, for any reconstructor $\Psi$ with 1-accuracy $\eta_1^{-1} > 0$, there exists $\mathcal{E}^2_{\Psi}(\eta_1)$ such that $|| \x^*_{GT, 0} - \x^*_{\Psi, 0} ||_1 < \mathcal{E}^2_{\Psi}(\eta_1)$. This concludes the proof.
% \end{proof}
